CREIME: A Convolutional Recurrent model for Earthquake Identification and Magnitude Estimation

The detection and rapid characterisation of earthquake parameters such as magnitude are of prime importance in seismology, particularly in applications such as Earthquake Early Warning (EEW). Traditionally, algorithms such as STA/LTA are used for event detection, while frequency or amplitude domain parameters calculated from 1-3 seconds of first P-arrival data are sometimes used to provide a first estimate of (body wave) magnitude. Owing to extensive involvement of human experts in parameter determination, these approaches are often found to be insufficient. Moreover, these methods are sensitive to the signal to noise ratio and may often lead to false or missed alarms depending on the choice of parameters. We, therefore, propose a multitasking deep learning model the Convolutional Recurrent model for Earthquake Identification and Magnitude Estimation (CREIME) that: (i) detects the first earthquake signal, from background seismic noise, (ii) determines first P arrival time as well as (iii) estimates the magnitude using the raw 3-component waveform data from a single station as model input. Considering, speed is of essence in EEW, we use up to two seconds of P-wave information which, to the best of our knowledge, is a significantly smaller data window (5 second window with up to of P wave data) compared to the previous studies. To examine the robustness of CREIME we test it on two independent datasets and find that it achieves an average accuracy of 98 percent for event vs noise discrimination and is able to estimate first P arrival time and local magnitude with average root mean squared errors of 0.13 seconds and 0.65 units, respectively. We also compare CREIME architecture with architectures of other baseline models, by training them on the same data, and also with traditional algorithms such as STA/LTA, and show that our architecture outperforms these methods.

==> authors.tex <==
\author[fias,geo]{Megha Chakraborty} 
\author[fias,unimainz]{Darius Fenner}
\author[fias]{Wei Li} 
\author[fias,phys]{Johannes Faber} 
\author[fias, phys]{Kai Zhou}
\author[fias,geo]{Georg Rümpker}
\author[fias,phys,gsi]{Horst Stöcker} 
\author[fias]{Nishtha Srivastava} 
\ead{srivastava@fias.uni-frankfurt.de}

\affiliation[fias]{
    organization = {Frankfurt Institute for Advanced Studies},
    postcode = {60438},
    city = {Frankfurt am Main},
    country = {Germany}
}

\affiliation[geo]{
    organization = {Institute of Geosciences, Goethe-University Frankfurt},
    postcode = {60438},
    city = {Frankfurt am Main},
    country = {Germany}
}

\affiliation[phys]{
    organization = {Institute for Theoretical Physics, Goethe Universität},
    postcode = {60438},
    city = {Frankfurt am Main},
    country = {Germany}
}

\affiliation[gsi]{
    organization = {GSI Helmholtzzentrum für Schwerionenforschung GmbH},
    postcode = {64291}, 
    city = {Darmstadt},
    country = {Germany}
}

